Learning for Layered Safety-Critical Control with Predictive Control Barrier Functions

Safety filters leveraging control barrier functions (CBFs) are highly effective for enforcing safe behavior on complex systems. It is often easier to synthesize CBFs for a Reduced order Model (RoM), and track the resulting safe behavior on the Full order Model (FoM) -- yet gaps between the RoM and FoM can result in safety violations. This paper introduces \emph{predictive CBFs} to address this gap by leveraging rollouts of the FoM to define a predictive robustness term added to the RoM CBF condition. Theoretically, we prove that this guarantees safety in a layered control implementation. Practically, we learn the predictive robustness term through massive parallel simulation with domain randomization. We demonstrate in simulation that this yields safe FoM behavior with minimal conservatism, and experimentally realize predictive CBFs on a 3D hopping robot.

==> figurediagram.tex <==

% ____________________________ NOT WRAPPED FIGURE _________________________________________
\begin{figure}
  \begin{center}
  \begin{footnotesize}
  \begin{tikzpicture}[
  mynode/.style = {draw, text width=0.45\textwidth, align=center, minimum height=0.8cm}]

  %%%Nodes
    \node[mynode] (high) {\textbf{Reduced order Model (RoM)}
    \begin{align} %\label{eq:decision-layer}
    \begin{array}{rl}
   \textrm{Dynamics:} \quad  & \dot{\b z}_t = \b f(\b z_t) + \b g(\b z_t) \b v_t, \\ 
   \textrm{Safety:} \quad  & h(\b z_t) \geq 0, \quad \forall t \geq 0.
    \end{array} \nonumber
    \end{align}
    };
    
    \node[mynode, below=of high] (mid) {\textbf{Predictive CBF}
\begin{align}
\b k_{sf}^{\delta}(\b z, \b x) = & \argmin _{\b v \in \cal V}   \quad \frac{1}{2}\| \b v - \b k(\b z) \|^2 \nonumber\\
\mathrm{s.t.} \quad  &   \L_f h(\b z)  + \L_g h(\b z)  \b v \geq -\alpha h(\b z) + \delta(\b x) \nonumber
\end{align}
    };
    
    \node[mynode, below=of mid] (low) {\textbf{Full order Model (FoM)}
    \begin{align}
    \begin{array}{rl}
   \textrm{Dynamics:} \quad  & \dot{\b x}_t =  \bF (\bx_t) + \bG(\bx_t) \b K(\b x_t,\b v_t), \\ 
   \textrm{Safety:} \quad  & h(\Pi(\b x_t)) \geq 0, \quad \forall t \geq 0.
    \end{array} \nonumber
    \end{align}
    };


         \begin{scope}[transform canvas={xshift=.6em}]
    \draw[latex-] (high) --  node[right] {$ 
    \begin{array}{l} \textbf{Top Interface} \\ 
\b v_t = \b k_{sf}^{\delta}(\b z_t, \b x_t)
\end{array}
$  }  ++  (mid);
    \end{scope}
    \begin{scope}[transform canvas={xshift=-.6em}]
    \draw[-latex] (high) --  node[left] {$\b z_t $  }  ++  (mid);
    \end{scope}
    
    % \begin{scope}[transform canvas={xshift=.4em}]
    % \draw[latex-latex] (high) --  node[right] {$ 
    % \begin{array}{l} \textbf{Top Interface} \\ 
    % r(k) \in s(\lfloor k/\delta\rfloor) 
    % \end{array}
    % $  }  ++  (mid);
    % \end{scope}
    % \begin{scope}[transform canvas={xshift=-.4em}]
    % \draw[-latex] (mid) --  node[left] {$r(k)$  }  ++  (high);
    % \end{scope}

    %     \draw[latex-latex] (mid) --  node[right] {$ 
    % \begin{array}{l} \textbf{Bottom Interface} \\ 
    % r(k) = x(k) \\
    % x(k)=x_{k\tau},\forall k\in\mathbb N
    % \end{array}
    % $  }  ++  (low);

  \begin{scope}[transform canvas={xshift=.6em}]
        \draw[-latex] (mid) --  node[right] {$ 
    \begin{array}{l} \textbf{Bottom Interface} \\ 
\b v_t = \b k_{sf}^{\delta}(\b z_t, \b x_t)
\end{array}
$  }  ++  (low);
    \end{scope}
    \begin{scope}[transform canvas={xshift=-.6em}]
    \draw[latex-] (mid) --  node[left] {$\b x_t $ }  ++  (low);
    \end{scope}


     \draw [latex-latex] (low.west) -- ++(-1cm,0) |- (high)
 node[pos=0.25,sloped,above]{State Projection: $z = \Pi(x)$};

     % \draw [-latex] (low.west) -- ++(-0.5cm,0) |- (mid)node[pos=0.25,sloped,above]{$r(0) =  x(0) = x_0$};;

         \draw [latex-latex] (low.east) -- ++(1cm,0) |- (high)
 node[pos=0.25,sloped,below]{Input Projection: $v = \Psi(x)$};
    
  \end{tikzpicture}
  \vspace{-.4cm}
  \end{footnotesize}
  \end{center}
  \caption{The layered architecture of a RoM and FoM interacting through a Predictive CBF.}
  \label{fig:architecture}
\end{figure}
% ____________________________ END NOT WRAPPED FIGURE _________________________________________

